From Complexity to Simplicity: Adaptive ES-Active Subspaces for Blackbox Optimization

We present a new algorithm ASEBO for optimizing high-dimensional blackbox functions. ASEBO adapts to the geometry of the function and learns optimal sets of sensing directions, which are used to probe it, on-the-fly. It addresses the exploration-exploitation trade-off of blackbox optimization with expensive blackbox queries by continuously learning the bias of the lower-dimensional model used to approximate gradients of smoothings of the function via compressed sensing and contextual bandits methods. To obtain this model, it leverages techniques from the emerging theory of active subspaces in the novel ES blackbox optimization context. As a result, ASEBO learns the dynamically changing intrinsic dimensionality of the gradient space and adapts to the hardness of different stages of the optimization without external supervision. Consequently, it leads to more sample-efficient blackbox optimization than state-of-the-art algorithms. We provide theoretical results and test ASEBO advantages over other methods empirically by evaluating it on the set of reinforcement learning policy optimization tasks as well as functions from the recently open-sourced Nevergrad library.

==> related_work.tex <==

\section{Related Work}\label{sec:related_work}

There have been a variety of works seeking to reduce sampling complexity for ES methods through the use of metric learning. In particular, the covariance matrix adaptation evolution strategy (CME-ES) is a state-of-the-art derivative free blackbox optimization algorithm, which seeks to learn and maintain a fully parameterized Gaussian distribution. In typical blackbox optimization settings the function evaluation is the bottleneck, however, CMA-ES suffers from quadratic time complexity for each evaluation which can be limiting for high dimensional problems. As such, a series of attempts have been made to produce scalable variants of CMA-ES, by restricting the covariance matrix to the diagonal (sep-CMA-ES [1]) or a low rank approximation (VD-CMA-ES [2], LM-CMA-ES [3]). Two recent algorithms, VkD-CMA-ES [4] and LM-MA-ES [5], seek to combine the above ideas and have been shown to be successful in large-scale settings, including RL policy learning [6]. Although these methods are able to quickly learn and adapt the covariance matrix, they are heavily dependent on hyper-parameter selection [4,7] and lack a means to avoid learning a bias. As we show in section 5 with our experimental results, this bias is a severe limitation of existing approaches for metric learning.

(I have these citations, will add to bib if we want to keep).


==> theory.tex <==
\vspace{-3mm} 
\section{Theoretical Results}\label{sec:theory}

In this section we provide theoretical guarantees for the ASEBO sampling mechanism, where sensing directions $\{ \mathbf{g}_i\}$ at time $t$ are sampled from the distribution
used in version $\mathbf{V2}$ of Algorithm 1:
\begin{equation*}
    \widehat{P} = \begin{cases}
            \mathbf{g} \sim \mathcal{N}(0, \mathbf{I}_{\mathcal{L}_{\mathrm{active}}}) & \text{ with probability } p^t \\
            \mathbf{g} \sim \mathcal{N}(0, \mathbf{I}_{\mathcal{L}_{\mathrm{active}}^\perp} ) & \text{ with probability } 1-p^t,
        \end{cases}
\end{equation*}
where $p^t$ is a probability parameter with values in $[0,1]$.
%\subsection{Definitions and Assumptions}


Following notation in Algorithm 1, denote by $\mathbf{U}^{\mathrm{act}} \in \mathbb{R}^{d\times r}$ a 
matrix obtained by stacking together vectors of some orthonormal basis of $\mathcal{L}^{\mathrm{ES}}_{\mathrm{active}}$,
where $\mathrm{dim}(\mathcal{L}^{\mathrm{ES}}_{\mathrm{active}}) = r$ and by $\mathbf{U}^{\perp} \in \mathbb{R}^{d\times (d-r)}$
a matrix obtained from stacking together vectors of some orthonormal basis of its orthogonal complement $\mathcal{L}^{\mathrm{ES}, \perp}_{\mathrm{active}}$.
Denote by $\sigma$ a smoothing parameter.

We make the following regularity assumptions on $F$:
\begin{itemize}
    \item[] \textbf{Assumption 1}. $F$ is $L-$Lipschitz, i.e. for all $\theta, \theta' \in \mathbb{R}^d$, $|F(\theta) - F(\theta')| \leq L \| \theta - \theta'\|_{2}$ for some $L>0$.
    \item[] \textbf{Assumption 2}. $F$ has a $\tau$-smooth third order derivative tensor with respect to $\sigma>0$, 
    so that $F(\theta + \sigma \mathbf{g}) = F(\theta) + \sigma \nabla F(\theta)^\top 
    \mathbf{g} + \frac{\sigma^2}{2}\mathbf{g}^\top H(\theta )\mathbf{g} + \frac{1}{6} \sigma^3 F'''(\theta)[\mathbf{v},\mathbf{v},\mathbf{v}]$ 
    for some $\mathbf{v} \in \mathbb{R}^{d}$ ($\|\mathbf{v}\|_{2} \leq \|\mathbf{g}\|_{2}$) 
    satisfying  $|F'''(\theta)[\mathbf{v},\mathbf{v},\mathbf{v}] \leq \tau \|\mathbf{v} \|_{2}^3 \leq \tau \| \mathbf{g}\|_{2}^3$.
\end{itemize}

Under these assumptions, the one-sample baseline antithetic estimator 
$\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)$ of $\nabla F_{\sigma}(\theta)$ given as: 
$\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta) := \frac{F(\theta + \sigma \mathbf{g}) \mathbf{g} + F(\theta + \sigma \mathbf{g})(-\mathbf{g})}{2\sigma}$
for $\mathbf{g} \sim \mathcal{N}(0,\mathbf{I}_{d})$
satisfies  $\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta) = \mathbf{g}\mathbf{g}^\top \nabla F(\theta) + \xi_\mathbf{g}(\theta)\mathbf{g}$ 
such that $|\xi_\mathbf{g}(\theta) |\leq \tau\sigma^2 \| \mathbf{g}\|_{2}^3$. 
An analogous statement is true for the corresponding $\mathrm{ASEBO}$ one-sample estimator corresponding to sensings sampled from $\widehat{P}$. 
Observe also that the following is true:
\begin{equation*}
      \mathbb{E}_{\mathbf{g} \sim \widehat{P} } \left[   \mathbf{g}\mathbf{g}^\top         \right] = \underbrace{\left( p^t \mathbf{U}^{\mathrm{act}}\left(\mathbf{U}^{\mathrm{act}}   \right)^\top + (1-p^t) \mathbf{U}^{\perp}\left(  \mathbf{U}^{\perp} \right)^\top \right)}_{\mathbf{C}_1} 
\end{equation*}
% \begin{equation*}
%     \mathbb{E}_{\mathbf{g} \sim P_i } \left[   \mathbf{g}\mathbf{g}^\top         \right] =  \begin{cases}
%                                    \underbrace{\left( p_t VV^\top + (1-p_t) V_\perp V_\perp^\top          \right)}_{C_1} & \text{if } P_1 \\
%                                    \underbrace{\left(  p_t VV^\top + I   \right)}_{C_2}  & \text{if } P_2
%                                                      \end{cases}
% \end{equation*}

Let $\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta) = \mathbf{C}_1^{-1} \frac{F(\theta + \sigma \mathbf{g})\mathbf{g} + F(\theta + \sigma \mathbf{g}) (-\mathbf{g})}{2\sigma} $ 
be the gradient estimator corresponding to $\widehat{P}$ (we tested empirically that the inverse covariance renormalization factor $\mathbf{C}_1^{-1}$ does not change learning profiles in practice,
but we incorporate it here since it is needed for rigorous theoretical analysis). 
We start by showing that under the assumption of noiseless evaluation of $F$, both the bias of $\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)$ 
and the bias of $\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)$ are small.  Let $\epsilon > 0$. 
Throughout this section we will assume that $\sigma$ is small enough, i.e. $\sigma < \frac{1}{35}\sqrt{\frac{\epsilon \min(p^t, 1-p^t)}{\tau  d^3 \max(L, 1)} }$ for some precision parameter $\epsilon > 0$.

\begin{lemma}\label{lemma::gradients_approximation}
If $F$ satisfies Assumptions 1 and 2, the gradient estimators $\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)$ and 
$\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)$ satisfy:
\begin{align*}
    \left \| \mathbb{E}_{\mathbf{g} \sim \mathcal{N}(0, \mathbf{I}_{d})}\left[  \widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)\right] - \nabla F(\theta) \right \| &\leq \epsilon \\
    \left \| \mathbb{E}_{\mathbf{g} \sim \widehat{P}}\left[  \widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)\right] - \nabla F(\theta) \right \| &\leq\epsilon
\end{align*}
Consequently $\mathbb{E}_{\mathbf{g} \sim \mathcal{N}(0, \mathbf{I}_{d})} \left[ \mathbf{U}^{\mathrm{act}}(\mathbf{U}^{\mathrm{act}})^\top \widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)  \right] \approx \left( \nabla F(\theta_t)     \right)_{\mathrm{active}}$ and 
$\mathbb{E}_{\mathbf{g} \sim \widehat{P}} \left[ \mathbf{U}^{\mathrm{act}}(\mathbf{U}^{\mathrm{act}})^\top \widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)   \right] \approx \left( \nabla F(\theta_t)     \right)_{\mathrm{active}}$ and 
analogous statements hold for $\mathbf{U}^{\perp}$.
\end{lemma}



% Consider $\left(   VV^\top C_i^{-1}\mathbf{g}\mathbf{g}^\top \nabla F(\theta_t)    \right)^\top (VV^\top C_i^{-1}\mathbf{g}\mathbf{g}^\top \nabla F(\theta_t) ) = 
% \nabla F(\theta_t)^\top \mathbf{g}\mathbf{g}^\top C_i^{-1} VV^\top VV^\top C_i^{-1} \mathbf{g}\mathbf{g}^\top \nabla F(\theta_t) = \nabla F(\theta_t)^\top 
% \mathbf{g}\mathbf{g}^\top C_i^{-1} VV^\top C_i^{-1} \mathbf{g}\mathbf{g}^\top \nabla F(\theta_t) $.

% The inverse of $C_i$ can be written as:

% \begin{equation*}
%     C_i^{-1} = \begin{cases}
%                 \frac{1}{p_t} VV^\top + \frac{1}{1-p_t} V_\perp V_\perp^\top & \text{if } P_1 \\
%                 \frac{-p_t}{1+p_t}VV^\top + I & \text{if } P_2
%                 \end{cases}
% \end{equation*}

% And therefore:

% \begin{equation*}
%     \mathbb{E}_{\mathbf{g} \sim P_i}\left[    \nabla F(\theta_t)^\top \mathbf{g}\mathbf{g}^\top C_i^{-1} VV^\top C_i^{-1} \mathbf{g}\mathbf{g}^\top \nabla 
% F(\theta_t)  \right]  = \begin{cases}
               
%                 \end{cases}
% \end{equation*}
\subsection{Estimating ratio $r$ for ``exploring how to explore''}
In this section we provide guarantees for the estimation of the ratio $r$ as specified in Equation \ref{eq::ratio} for
Algorithm \ref{Alg:uniform_sampling}. 


Let $s_{\mathbf{U}^{\mathrm{act}}} = \| (\mathbf{U}^{\mathrm{act}})^\top \nabla F(\theta)  \|_{2}^2$ and 
    $s_{\mathbf{U}^{\perp}}  = \|  (\mathbf{U}^{\perp})^\top \nabla F(\theta)  \|_{2}^2 $. The results of this section hinge on the observation that 
whenever $\mathbf{g} \sim \mathcal{N}(0, \mathbf{I}_{\mathcal{L}^{\mathrm{ES}}_{\mathrm{active}}})$  
the distribution of $\frac{F(\theta + \sigma \mathbf{g}) - F(\theta - \sigma \mathbf{g})}{2\sigma} \approx N(0, s_{\mathbf{U}^{\mathrm{act}}})$. 
Analogously when  $\mathbf{g} \sim \mathcal{N}(0, \mathbf{I}_{\mathcal{L}_{\mathrm{active}}^{\mathrm{ES},\perp}})$ the distribution of 
$\frac{F(\theta_t + \sigma \mathbf{g}) - F(\theta_t - \sigma \mathbf{g})}{2\sigma} \approx N(0, s_{\mathbf{U}^{\perp}} )$. 
The next theorem quantifies how large horizon $C$ from both theorems should be to obtain a good empirical approximation for the ratio $r$.   
\begin{theorem}
Let $0<s<C$ and
let $\mathbf{g}_i \sim \mathcal{N}(0, \mathbf{I}_{\mathcal{L}^{\mathrm{ES}}_{(\mathrm{active})}})$
for $i=1,...,s$ and $\mathbf{g}_{i}, \sim \mathcal{N}(0, \mathbf{I}_{\mathcal{L}_{\mathrm{active}}^{\mathrm{ES}, \perp}})$ for $i=s+1,...,C$. 
Let $\hat{s}_{\mathbf{U}^{\mathrm{act}}} := \frac{1}{s}\sum_{j=1}^s \left(  \frac{F(\theta + \sigma \mathbf{g}_j) - F(\theta - \sigma \mathbf{g}_j) }{2\sigma} \right)^2$, $\hat{s}_{\mathbf{U}^{\perp}}  
:=\frac{1}{C-s} \sum_{j=1}^{C-s} \left( \frac{F(\theta + \sigma \mathbf{g}_j) - F(\theta - \sigma \mathbf{g}_j) }{2\sigma}\right)^2$ and let $\hat{r} = 
\sqrt{\frac{\hat{s}_{\mathbf{U}^{\mathrm{act}}} }{\hat{s}_{\mathbf{U}^{\perp}}}} $. Given $u, \epsilon > 0$ and $\delta  \in (\epsilon,1)$, the following holds.
\begin{enumerate}
\item If $C = 2s$ for $s \geq \frac{16}{u^2}\log\left(\frac{8}{\delta}\right)$ and under the mechanism from Algorithm \ref{Alg:uniform_sampling} or
\item If $\{ \mathbf{g}_i \}_{i=1}^C$ are samples generated under $\widehat{P}$,  $\min(p^t, 1-p^t) > u$ and $C \geq \max\left(  \frac{8}{(p^t-u) u^2 }  ,   
\frac{8}{(1-p^t-u)u^2}, \frac{2p^t + 2u/3}{u^2}  \right) \log\left(  \frac{12}{\delta}     \right)$, 
\end{enumerate}
then with probability at least $1-\delta$:
\begin{equation*}
    \sqrt{\frac{s_{\mathbf{U}^{\mathrm{act}}}(1-u) - \frac{2\epsilon}{\delta} }{ s_{\mathbf{U}^{\perp}}(1+u) + \frac{2\epsilon}{\delta}  } }  \leq \widehat{r} \leq \sqrt{\frac{s_V(1+u) + \frac{2\epsilon}{\delta} }{ s_{V^\perp}(1-u) - \frac{2\epsilon}{\delta}}}.
\end{equation*}
\end{theorem}

\subsection{Variance reduction via non isotropic sampling}
We show now that under the sampling strategy encoded by distribution $\widehat{P}$, the variance of the gradient estimator can be made smaller by choosing the probability parameter $p^t$ appropriately. 
We conclude that given an appropriate subspace partition $\mathcal{L}^{\mathrm{ES}}_{\mathrm{active}}, \mathcal{L}^{\mathrm{ES},\perp}_{\mathrm{active}}$ and the right choice of $p^t$, the variance of $\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)$ can 
be orders of magnitude smaller than the variance of $\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)$. Denote: $d_{\mathrm{active}} = \mathrm{dim}(\mathcal{L}_{\mathrm{active}}^{\mathrm{ES}})$ and $d_{\perp} = \mathrm{dim}(\mathcal{L}_{\mathrm{active}}^{\mathrm{ES}, \perp})$.
The following holds:
%The later can be written as:
\begin{lemma}\label{lemma:variance_z1}
The variance of ${\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)}$ satisfies:
\begin{equation*}
| \mathrm{Var}[{\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)}] - \Gamma | \leq \epsilon
\end{equation*}
for $\Gamma = \frac{d_{\mathrm{active}}+2}{p^t} s_{\mathbf{U}^{\mathrm{act}}} - \frac{d_{\perp} + 2}{1-p^t} s_{\mathbf{U}^{\perp}} + \|\nabla F(\theta)\|^2$.

\end{lemma}
The choice of $p^t$ that minimizes $\Gamma$ equals:
\begin{equation*}
    p^t_* = \frac{ \sqrt{ (s_{\mathbf{U}^{\mathrm{act}}})(d_{\mathrm{active}} + 2) } }{   \sqrt{(s_{\mathbf{U}^{\mathrm{act}}})(d_{\mathrm{active}} + 2)} +  \sqrt{(s_{\mathbf{U}^{\perp}})(d_{\mathbf{U}^{\perp}} + 2)}}.  
\end{equation*}
\begin{lemma}
The optimal variance $\mathrm{Var}_{\mathrm{opt}}$ corresponding to $p^t_*$ satisfies:
$|\mathrm{Var}_{\mathrm{opt}} - \Delta| \leq \epsilon$ 
for $\Delta =      \left[  \sqrt{(s_{\mathbf{U}^{\mathrm{act}}})(d_{\mathrm{active}} + 2)} +    \sqrt{(s_{\mathbf{U}^{\perp}})(d_{\perp} + 2)} \right]^2 - \| \nabla F(\theta) \|^2$.
\end{lemma}

Our main theoretical result in this subsection states that:

\begin{theorem}\label{theorem::variance_reduction_p1}
$\mathrm{Var}_{\mathrm{opt}} \leq \mathrm{Var}[{\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)}] + \epsilon - \lambda$ where
\begin{align*}
  \lambda &:= | \sqrt{(s_{\mathbf{U}^{\perp}})(d_{\mathrm{active}} + 2)} -  \sqrt{(s_{\mathbf{U}^{\mathrm{act}}})(d_{\perp} + 2)}  |^2- \\
  &2 \| \nabla F(\theta)\|^2.
\end{align*}
The slack $\lambda$ is always nonnegative. The inequality is strict, for example when $s_{\mathbf{U}^{\perp}}  = 0$ and $d_{\perp}  \geq 1$. In this case $\mathrm{Var}[{{\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)}}] \approx (d+1)\| \nabla F(\theta)\|^2$ 
whereas $\mathrm{Var}_{\mathrm{opt}} \approx (d_{\mathrm{active}} + 1)\| \nabla F(\theta) \|^2$. Thus achieved gains can be substantial. 
\end{theorem}



\subsection{Adaptive Mirror Descent}
In Theorem \ref{theorem::variance_reduction_p1} we proved that for appropriate choices of $\mathcal{L}^{\mathrm{ES}}_{\mathrm{active}}$ and $p_{t}$, 
gradient estimator ${\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)}$ will have
significantly smaller variance than ${\widehat{\nabla}^{\mathrm{AT},\mathrm{base}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)}$. 
In this section we show that Algorithm \ref{Alg: exponentiated_sampling} provides an adaptive way to choose $p^t$. 
Using tools from contextual bandits theory, we provide regret guarantees that quantify the rate at which this 
Algorithm \ref{Alg: exponentiated_sampling} minimizes the variance of ${\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)}$ 
and converges to the optimal $p^t_*$.

Let $\mathbf{p}^t_{l} = \binom{p^t_{l}}{1-p^t_{l}}$. The main component $\Gamma$ of 
the variance of ${\widehat{\nabla}^{\mathrm{AT},\mathrm{asebo}}_{\mathrm{MC},k=1}F_{\sigma}(\theta)}$ as a function of $\mathbf{p}^t_l$ equals (Lemma \ref{lemma:variance_z1}) :
\begin{equation*}
\Gamma = \ell(\mathbf{p}^t_l) =\frac{d_{\mathrm{active}} + 2}{\mathbf{p}^t_l(1)} s_{\mathbf{U}^{\mathrm{act}}} + \frac{ d_{\perp} +2}{\mathbf{p}^t_l(2)} s_{\mathbf{U}^{\perp}} - \|\nabla F(\theta) \|^2.
\end{equation*}
The gradient $\nabla_{\mathbf{p}^t_l} \ell(\mathbf{p}^t_l)$ satisfies:
\begin{equation*}
    \nabla_{\mathbf{p}^t_l}  \ell(\mathbf{p}^{t}_{l}) = \binom{-\frac{d_{\mathrm{active}} + 2}{(\mathbf{p}^{t}_{l}(1))^2} 
    s_{\mathbf{U}^{\mathrm{act}}} }{ -\frac{d_{\perp} + 2}{(\mathbf{p}^{t}_{l}(2))^2} s_{\mathbf{U}^{\perp}}}  = 
    \mathbb{E}\left[ \binom{-\frac{a^t_l(d_{\mathrm{active}} + 2)}{(\mathbf{p}^{t}_{l}(1))^3}  }{ -\frac{(1-a^t_l)(d_{\perp} + 2)}{(\mathbf{p}^{t}_{l}(2))^2} } v_l^2    \right],
\end{equation*}
where $a^t_l, v_{l}$ are defined as in Algorithm \ref{Alg: exponentiated_sampling}.
\begin{theorem}
If $F$ satisfies Assumptions 1 and 2, 
$\sigma < \frac{1}{35}\sqrt{\frac{\epsilon \min(p^t, 1-p^t)}{\tau  d^3 \max(L, 1)} }$, $\alpha = \frac{2\beta^2}{\sqrt{C}\sqrt{   (d_{\mathrm{active}}+2)^2 s_{\mathbf{U}^{\mathrm{act}}}^2+(d_{\mathrm{\perp}}+2)s_{\mathbf{U}^{\perp}}^2 }}$ and $\epsilon = \frac{\beta^3}{2C (d+1)}$ then  Algorithm \ref{Alg: exponentiated_sampling} satisfies:
% \begin{equation*}
%   \frac{1}{C}\left[ \sum_{l=1}^C \ell(\mathbf{p}_t^l) \right] - \min_{\mathbf{p} \in \Delta_2} \ell(\mathbf{p})  \leq \frac{1}{\sqrt{C}} 
% \end{equation*}
\begin{equation*}
    \frac{1}{C}\mathbb{E}\left[  \sum_{l=1}^C   \ell(\mathbf{p}^t_l  )  \right]  -\min_{\mathbf{p} \in \beta + (1-2\beta)\Delta_2} \ell(\mathbf{p}) \leq \frac{\mathrm{Var}_{\mathrm{opt}}}{\beta^2 \sqrt{C}}+ \frac{1}{C}
\end{equation*}
Where $\Delta_2$ denotes the two dimensional simplex.
\end{theorem}



%  \begin{proof}
%  By concentration of squared gaussian random variables:
%         \begin{align*}
%             \mathbb{P}\left[ | \hat{s}_{V} -  s_V | \geq u s_V     \right] \leq 2\exp\left(-\frac{s u^2}{8}\right)  \\
%             \mathbb{P}\left[     | \hat{s}_{V^\perp} -  s_{V^\perp} | \geq u s_{V^\perp}   \right] \leq 2\exp\left( -\frac{(k-s)u^2}{8} \right)
%         \end{align*}
% Consequently, with probability $1-2\exp\left(  -\frac{su^2}{8}  \right) - 2\exp\left(  -\frac{(k-s)u^2}{8} \right)$, it holds that:
% \begin{equation*}
%     \frac{s_V}{s_{V^\perp}}\left( \frac{1+u}{1-u}    \right) \geq \frac{\hat{s}_V}{\hat{s}_{V^\perp}} \geq \frac{s_V}{s_{V^\perp}} \left( \frac{1-u }{1+u} \right)
% \end{equation*}
%     In fact, by \textcolor{red}{insert citation}, given $\epsilon >0$, $| s - kp_t  |\leq k\epsilon$ and $| (k-s) - (1-p_t)k | \leq k\epsilon$ with probability at 
% least $1 - \exp\left( -\frac{k\epsilon^2}{2p_t} \right) - \exp\left(   -\frac{k\epsilon^2 }{ 2p_t + 2\epsilon/3 }\right)$. And therefore the result follows.
% \end{proof}
    
    
% When $\mathbf{g}\sim P_2$, the distribution of $\frac{F(\theta_t + \sigma \mathbf{g}) - F(\theta_t + \sigma \mathbf{g})}{2\sigma} \approx N(0,p_t \| V^\top 
% \nabla F(\theta_t) \|^2 + \| \nabla F(\theta_t)\|^2 )$.

% \begin{theorem}
% Let $\mathbf{g}_1, \cdots, \mathbf{g}_{k_1} \sim P_1$ and $\mathbf{g}_{k_1+1}, \cdots, \mathbf{g}_{k}\sim \mathcal{N}(0, \mathbb{I})$. Let $\hat{s}_1 = \frac{1}{k_1} 
% \sum_{j=1}^{k_1} \left( \mathbf{g}_j^\top \nabla F(\theta_t)   \right)^2$ and $\hat{s}_2 = \frac{1}{k-k_1} \sum_{j = k_1+1}^k \left(   \mathbf{g}_j^\top  \nabla F(\theta_t)   \right)^2$. 
% Define $\hat{s}_V :=\frac{1}{p_t}\left(  \hat{s}_1 - \hat{s}_2 \right)$ and $\hat{s}_{V^{\perp}}:= \frac{(1+p_t) \hat{s}_2 - \hat{s}_1}{p_t}$. Given $\epsilon > 0, u > 0$, 
% with probability\textcolor{red}{ Write the correct concentration bound. Similar to above.}: 
% \begin{equation*}
%     \frac{s_V}{s_{V^\perp}}\left( \frac{1+u}{1-u}    \right) \geq \frac{\hat{s}_V}{\hat{s}_{V^\perp}} \geq \frac{s_V}{s_{V^\perp}} \left( \frac{1-u }{1+u} \right)
% \end{equation*}    
% \end{theorem}

% \begin{proof}
% \textcolor{red}{Write proof. Sum of subexponential random variables, etc .... }
% \end{proof}









% \subsection{Approximating $r$ via compressed sensing and contextual bandits}
% \label{sec:jlt_bandits}
